Lifted Probabilistic Inference for Asymmetric Graphical Models

Lifted probabilistic inference algorithms have been successfully applied to a large number of symmetric graphical models. Unfortunately, the majority of real-world graphical models is asymmetric. This is even the case for relational representations when evidence is given. Therefore, more recent work in the community moved to making the models symmetric and then applying existing lifted inference algorithms. However, this approach has two shortcomings. First, all existing over-symmetric approximations require a relational representation such as Markov logic networks. Second, the induced symmetries often change the distribution significantly, making the computed probabilities highly biased. We present a framework for probabilistic sampling-based inference that only uses the induced approximate symmetries to propose steps in a Metropolis-Hastings style Markov chain. The framework, therefore, leads to improved probability estimates while remaining unbiased. Experiments demonstrate that the approach outperforms existing MCMC algorithms.

==> figs/fixbb <==
#!/bin/bash

# This is fixbb version 0.31.  Copyright 2000 by Jeff Spirko.
# Redistributable under the GNU General Public License.
# See http://topquark.dhs.org/~spirko/fixbb/

# Changes by Petr Mikulik:
#   -  8.  9. 2000: working file in the $TMP directory; remove backup file
#   - 18. 10. 2000: AWKPARSEBB to support multiple-page (non-EPS) documents
#   - 26. 10. 2000: error if bounding box not determined (GS < 5.50 or empty
#     pages); page status info added

# Options for ghostscript to print the BoundingBox without other junk.
GSOPTS="-dQUIET -dBATCH -dNOPAUSE -sDEVICE=bbox"
export GSOPTS

# Original awk program, checks each line of the file
#AWKPROG='{ if ($1 == "%%BoundingBox:") 
#  print $1, ENVIRON["bbox"]; 
#  else print;}'

# Slightly faster version, doesn't bother looking after finding a BoundingBox.
# What happens if there is more than one BoundingBox?  Can this happen?
AWKPROG='
	(found) { print; next }
	$1 == "%%BoundingBox:" { print $1, ENVIRON["bbox"]; found=1; next }
	{ print }
	'

# Finds min and max of the 4 numbers after the "%%BoundingBox:" label
AWKPARSEBB='
	BEGIN { x1=99999; y1=99999; x2=0; y2=0; page=0 }
	$1!= "%%BoundingBox:" { next }
	$2<0 || $3<0 { next }
	x1>$2 { x1=$2 }
	y1>$3 { y1=$3 }
	x2<$4 { x2=$4 }
	y2<$5 { y2=$5 }
	{ page++; printf "Page " page ": " $0 "  max = " x1 " " y1 " " x2 " " y2  "  \t\r" >"/dev/stderr" }
	END { printf "\t\t\t\t\t\t\t\r" >"/dev/stderr"
	      print x1 " " y1 " " x2 " " y2 }
	'

export bbox

# Each command-line argument is assumed to be a file to process
for FILE in $* ; do

#  BAK=${FILE}~
#  if [ "$TMP" = "" ]; then TMP="."; fi; BAK=$TMP\fixbb__.ps
  BAK='fixbb$$.ps'

  # Get the correct BoundingBox from ghostscript.
  # Old: bbox=`gs ${GSOPTS} ${FILE} 2>&1 | gsort | head -1 | cut -d\  -f 2-`
  bbox=`/usr/bin/gs ${GSOPTS} ${FILE} 2>&1 | awk "$AWKPARSEBB"`

  case $bbox in
    "99999 99999 0 0")
	echo "Bounding box was NOT determined (empty pages or Ghostscript >= 5.50 required)"
	exit ;;
  esac

  echo "Bounding box for \""$FILE"\" is: "$bbox

  # Save the old version of the file
  mv $FILE $BAK

  # Create the new version, replacing the old BoundingBox
  awk "$AWKPROG" $BAK > $FILE

  case `uname` in 
    "OS/2") dos2unix $FILE ;;
  esac

  # delete the backup file
  rm -f $BAK

done

